Crowd Counting Using Scale-Aware Attention Networks

In this paper, we consider the problem of crowd counting in images. Given an image of a crowded scene, our goal is to estimate the density map of this image, where each pixel value in the density map corresponds to the crowd density at the corresponding location in the image. Given the estimated density map, the final crowd count can be obtained by summing over all values in the density map. One challenge of crowd counting is the scale variation in images. In this work, we propose a novel scale-aware attention network to address this challenge. Using the attention mechanism popular in recent deep learning architectures, our model can automatically focus on certain global and local scales appropriate for the image. By combining these global and local scale attention, our model outperforms other state-of-the-art methods for crowd counting on several benchmark datasets.

==> bar_shanghai.tex <==
\begin{figure}
\caption{Comparison of ACNN's predictions and ground truth counts for ShanghaiTech Part B dataset. \textbf{THIS CHART IS WRONG AND WILL BE REPLACED; GROUPS ARE NOT SUPPOSED TO FORM RANDOMLY.}}\label{part_B}
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.1,
    %/pgfplots/scaled y ticks=true,
    legend style={at={(0.75,0.97)},
      anchor=north,legend columns=-1,font=\small},
    ylabel={Total Count \#/Group},
    xlabel={Group},
    symbolic x coords={1,2,3,4,5,6,7,8,9,10},
    enlarge y limits={upper,value=0.5},%enlarges the plot area, so that bar values fit in.
    ymin=2500,
    width=13cm,
    height=6cm,
    /pgf/bar width=11pt,% bar width
    %xtick=data,
    nodes near coords,
    every node near coord/.append style={rotate=90, anchor=west},% rotate the numbers above the bars so the're no longer ugly;-)
    %nodes near coords align={vertical} style={rotate=90, anchor=east},
    ]
\addplot coordinates {(1,4254) (2,4428) (3,3411) (4,3628) (5,4596) (6,3504) (7,3436) (8,3461) (9,3542) (10,4157)};
\addplot coordinates {(1,3891) (2,4432) (3,3517) (4,3713) (5,4569) (6,3547) (7,3528) (8,3459) (9,3539) (10,3991)};
%\addplot coordinates {(tool8,1) (tool9,1) (tool10,1)};
\legend{Ground Truth,ACNN's Prediction}

\end{axis}
\end{tikzpicture}

\end{figure} 

==> experiment_presentation.tex <==
\section{Experiments}\label{sec:experiments}
We first introduce the datasets and our experimental setup. We then present experimental results on three benchmark datasets. Finally, we perform ablation studies to further analyze our proposed approach.

\subsection{Datasets and Setup}\label{sec:setup}
\noindent{\bf Datasets:} We evaluate our proposed method on three benchmark datasets: ShanghaiTech PartB~\cite{zhangY16_cvpr}, Mall dataset~\cite{mall} and UCF\_CC\_50 \cite{idrees13_cvpr}. Table~\ref{tab:dataset} shows various statistics of these datasets. The ShanghaiTech PartB dataset contains 716 where 400 images are for training and the other 316 ones for testing. The Mall dataset~\cite{mall} has 2000 frames captured from a shopping mall. The first 800 frames are used as training frames and the remaining 1200 frames are used for testing. The UCF\_CC\_50 dataset~\cite{idrees13_cvpr} contains a total of 50 images from web sources. Clearly, the limited number of images in these datasets raises the need for data augmentation in order to prepare the data for training a deep network. Consequently, we used data augmentation to address the issue. We followed the same data augmentation technique used in existing methods \cite{decidenet,idrees13_cvpr,zhangY16_cvpr,sam17_cvpr,sindagi17_iccv}.

\begin{table*}[!htbp]

\begin{center}
%  \resizebox{.9\textwidth}{!}{
  \begin{tabular}{ | c  c  c  c  c  c  c |}
    \hline
    \textbf{Dataset} & \textbf{Resolution} & \textbf{Images} & \textbf{Max} & \textbf{Min} & \textbf{Avg} & \textbf{Total} \\ \hline
    
    ShanghaiTech PartB & $1024\times768$ & 716 & 578 & 9 & 123.6 & 88,488 \\ %\hline
    Mall & $320\times640$ & 2000 & 53 & 13 & 33 &  62325 \\ %\hline    
    UCF\_CC\_50 & varies & 50 & 4543 & 94 & 1279.5 & 63,974 \\ %\hline
    \hline
  \end{tabular}
%  }
%  \vspace{.4cm}
  \caption{Statistics of the three datasets used in the experiments. For each dataset, we show the following information: the image resolution, the number of images, the maximum/minimum number of people in an image, the average and total number of people annotated in the dataset.}
  \label{tab:dataset}  
\end{center}
\end{table*}
\noindent {\bf Evaluation Metric}: Following previous work \cite{zhangC15_cvpr,zhangY16_cvpr,sam17_cvpr,sindagi17_iccv,sindagi17_avss}, we use Mean Absolute Error (MAE) and Mean Square Error (MSE) as the evaluation metrics. Let $N$ be the number of test images, $\textrm{Count}_{gt}^{(n)}$ be the ground truth count and $\textrm{Count}^{(n)}$ be the predicted count for the $n$-th test image. These two evaluation metrics are defined as follows:
\begin{equation}
\text{MAE} =\frac{1}{N}\sum_{n=1}^{N} |Count^{(n)}-Count_{gt}^{(n)}|
\end{equation}
\begin{equation}
\text{MSE} =\sqrt[]{\frac{1}{N}\sum_{n=1}^{N} {|Count^{(n)}-Count_{gt}^{(n)}|}^2}
\end{equation}\\
\noindent {\bf Ground-truth Density Map}: On each dataset, head annotations (i.e. center of the head of a person) are provided as points. Following \cite{decidenet}, we generate the ground-truth density map from these point annotations by applying a Gaussian kernel normalized to have a sum of one.

%[[i removed ``training details'' since they are a bit too detailed. we can decide later on whether to keep some of them]]
\noindent {\bf Training Details:} We follow the data augmentation technique used in previous methods~\cite{decidenet,idrees13_cvpr,zhangY16_cvpr,sam17_cvpr,sindagi17_iccv}. Since there are lots of parameters in our model, directly learning all parameters from scratch is challenging. In our implementation, we use a two-phase training scheme to train our proposed model. During the first phase, we ignore the LSA module and only learn the parameters of the GSA, MFE, and FN modules. We assign each training image to one of three global scale classes (namely, low-density, mid-density, high-density) according to its ground-truth density map. We then learn the parameters of GSA, MFE, and FN modules by optimizing $L_{DM}+\lambda_{g}\cdot L_{GSA}$. During the second phase, we train all the modules (including LSA) together. The parameters of the GSA, MFE, and FN modules are initialized with the parameters obtained from the first phase. The parameters of the LSA module are initialized randomly from scratch.

%We follow the data augmentation technique used in existing methods \cite{decidenet,idrees13_cvpr,zhangY16_cvpr,sam17_cvpr,sindagi17_iccv}. We use a two-phase training scheme to train the proposed method. In the first phase, the ground truth density maps were arranged into three groups namely, low--dense, mid--dense, and high--dense samples. Although, arbitrary size of images are used to train MFE, we resized input images into $224\times224$ and fed it to GSA to generate attention scores $Score_i$ where $i$ is the number groups (Fig. \ref{fig:global}). These weights are then multiplied with three scale--aware outputs from MFE, respectively. Thus, this output dimension is ${W_i}/{4}\times{H_i}/{4}\times depth$. To take advantage of a pre--trained VGG16, we used fixed crop size of $224\times224$ and trained our GSA, MFE and FN networks in an end--to--end fashion. In phase 2 of training scheme, GSA, MFE and FN models which had been trained from phase 1 were used again to train LSA along with another round of training the whole network. The same dataset from phase 1 with arbitrary size of images are used to train LSA. Convolution with window size of  $64\times64$ are applied at the beginning of the LSA component (due to its effect in decreasing training time). Note that in phase 2, LSA was \textit{not} initialized from any pre--trained model and hence it learns its weights completely from scratch. The output of this network is 3 attention maps (Fig. \ref{fig:local}), namely $f_{j}$ ($ j = 1,2,3$) with size of ${W_i}/{4}\times{H_i}/{4}\times 1$ ($j$ is the density scale) each of which is associated with the output of one of MFE branches (Fig. \ref{fig:feature}). Finally, after being multiplied by global and local attention weights using Eq. \ref{eq:attention}, the outputs of three branches are stacked together and passed to FN to get final count.

\subsection{Experimental Results}\label{sec:results}
On the ShanghaiTech PartB dataset and the Mall dataset, we follow the standard training/testing split used in previous work~\cite{decidenet}. On the UCF\_CC\_50 dataset, we follow \cite{sindagi17_iccv} and perform 5-fold cross-validation. We apply the same data augmentation used in previous methods \cite{decidenet,idrees13_cvpr,zhangY16_cvpr,sam17_cvpr,sindagi17_iccv} on all datasets.

The experimental results on these three datasets are shown in Tables~\ref{shb_table}, Table~\ref{mall_table} and Table~\ref{ucf_table}, respectively. We also compare with existing state-of-the-art results on each of the datasets. On the ShanghaiTech PartB dataset and the Mall dataset, our proposed model significantly outperforms previous approaches in terms of both MAE and MSE. On the UCF\_CC\_50 dataset, our model outperforms previous approaches in terms of MAE. In terms of MSE, our model performs better than most previous approaches except for \cite{sindagi17_iccv}.

%From Table~\ref{shb_table}, we can see that proposed model outperforms all existing state-of-the-art approaches in terms of MAE and MSE. According to Table~\ref{tab:dataset}, Mall dataset contains comparatively less densed cowded images but the speciality of dataset is that all the images belong to a particular scene from a surveillance camera. From Table~\ref{mall_table}, its seen that proposed method outstrips all the state-of-the-art methods  on this particular scene based dataset (Mall). On UCF\_CC\_50, we outperform all the other approaches in terms of MAE (see Table~\ref{ucf_table}). In terms of MSE, we perform better than most previous methods except for \cite{sindagi17_iccv}. Figure \ref{fig:localatt} shows some qualitative examples of the density maps generated by our method.
\begin{table}[t]
\centering
%  \resizebox{.38\textwidth}{!}{
  \begin{tabular}{  |c  |c c|}
  \hline
    %\cline{2-3}
            Method & 
            \multicolumn{2}{c|}{\shortstack{ShanghaiTech\\Part B}}\\
            %\hline
             & MAE & MSE \\
            \hline
            %\hline
            R-FCN& 52.35 & 70.12  \\
            Faster R-CNN & 44.51 & 53.22 \\
            Cross-Scene& 32.00 & 49.80\\
            %\hline
            MC-CNN &26.40& 41.30\\
            %\hline
            Switching-CNN & 21.60 & 33.40  \\
            %\hline
            CP-CNN & 20.1 & 30.1 \\
            FCN & 23.76 & 33.12\\
            %\hline
            DecideNet & {20.75} & {29.42}  \\
            Ours & {\textbf{16.86}} & {\textbf{28.41}}  \\
            \hline
  \end{tabular}
%  }
%  \vspace{.4cm}
  \caption{Comparison of the performance of different methods on the ShanghaiTech PartB dataset~\cite{zhangY16_cvpr}. $^\dag$These results are obtained from \cite{decidenet}.}\label{shb_table}

\end{table}

\begin{table}[t]
\begin{center}
%  \resizebox{.38\textwidth}{!}{
  \begin{tabular}{  |c  |c c|}
  \hline
    %\cline{2-3}
            Method & 
             
            \multicolumn{2}{c|}{Mall}\\
            %\hline
             & MAE & MSE  \\
            \hline
            %\hline
            DecideNet & 1.52& 1.90 \\
            R-FCN&  6.02 & 5.46 \\
            Faster R-CNN &  5.91 & 6.60 \\
            SquareChn Detector & 20.55&439.10\\
            Count-Forest  & 4.40 &2.40 \\
            Exemplary-Density & 1.82 &2.74  \\
            Boosting-CNN  & 2.01& --\\
            %\hline
            Mo-CNN & 2.75 & 13.40 \\
            Weighted\_VLAD &2.41&9.12 \\
            %\hline
            Ours & {\textbf{1.28}} & {\textbf{1.68}} \\
            \hline
  \end{tabular}
%  }
%  \vspace{.4cm}
  \caption{Comparison of the performance of different methods on the Mall dataset~\cite{mall}. $^\dag$These results are obtained from \cite{decidenet}.}\label{mall_table}
\end{center}

\end{table}

\begin{table}[t]
\begin{center}
%  \resizebox{.38\textwidth}{!}{
  \begin{tabular}{  |c  |c c|}
  \hline
    %\cline{2-3}
            Method & 
            \multicolumn{2}{c|}{UCF\_CC\_50} \\
            %\hline
             & MAE & MSE  \\
            \hline
            %\hline
            Cross-Scene \cite{zhangC15_cvpr} &467.00 & 498.50 \\
            %\hline
            MC-CNN \cite{zhangY16_cvpr} & 377.60 & 509.10 \\
            %\hline
            Switching-CNN \cite{sam17_cvpr} &318.10 &439.20 \\
            %\hline
            CP-CNN \cite{sindagi17_iccv} & 295.80&{\bf320.90} \\
            Lempitsky et al. \cite{lempitsky10_nips}& 493.4&487.1  \\
            Idrees et al. \cite{idrees13_cvpr}& 419.5 & 541.6  \\
            %\hline
            Crowd-Net \cite{boominathan16_multimedia} &452.5&-- \\
            %\hline
            Hydra-2s \cite{rubio16_eccv}& 333.73 & 425.26\\
            %\hline
            Ours  &{\bf 271.60} & 391.00 \\
            \hline
  \end{tabular}
%  }
%  \vspace{.4cm}
  \caption{Comparison of the performance of different methods on the UCF\_CC\_50 dataset~\cite{idrees13_cvpr}.}\label{ucf_table}
\end{center}
\end{table}




\begin{figure*}[t]
  \centering
  {\setlength\tabcolsep{1pt}
  \begin{tabular}{cccc}
   
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_6.jpg}&
\includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/gt_6.png}&    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/14.jpg}&    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/gt_14.png}\\    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_12.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/gt_12.png}&    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/174.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/gt_174.png}\\
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_316.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/316.png}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1200.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1200.png}\\
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_315.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/315.png}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1199.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1199.png}\\    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_314.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/314.png}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1198.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1198.png}\\
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_313.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/313.png}&    
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1197.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1197.png}\\
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_312.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/312.png}& 
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1196.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1196.png}\\   
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_311.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/311.png}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1195.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1195.png}\\
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/IMG_299.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/299.png}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1194.jpg}&
    \includegraphics[width=1.4in,height=.84in]{qualitative_images/final_images/1194.png}\\
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/IMG_300.jpg}&
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/300.png}&
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/1193.jpg}&
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/1193.png}\\
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/IMG_301.jpg}&
    %includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/301.png}&
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/1192.jpg}&
    %\includegraphics[width=1.4in,height=.85in]{qualitative_images/final_images/1192.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_302.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/302.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1191.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1191.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_303.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/303.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1190.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1190.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_304.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/304.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1189.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1189.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_305.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/305.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1188.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1188.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_306.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/306.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1187.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1187.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_307.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/307.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1186.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1186.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_308.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/308.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1185.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1185.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_309.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/309.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1184.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1184.png}\\
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/IMG_310.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/310.png}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1183.jpg}&
    %\includegraphics[width=.85in,height=.67in]{qualitative_images/final_images/1183.png}\\
    
  \end{tabular}
  }
  \caption{Qualitative examples of density maps. The first two columns are original input images from the Shanghaitech partB \cite{zhangY16_cvpr} dataset and their corresponding density maps respectively. The last two columns are original input images from the Mall \cite{mall} dataset and their corresponding density maps respectively.}
  \label{fig:localatt}
\end{figure*}
%\vspace{-2.50cm}
\input{experiments_43_v3.tex}


